Learning with Neighbor Consistency for Noisy Labels

Recent advances in deep learning have relied on large, labelled datasets to train high-capacity models. However, collecting large datasets in a time- and cost-efficient manner often results in label noise. We present a method for learning from noisy labels that leverages similarities between training examples in feature space, encouraging the prediction of each example to be similar to its nearest neighbours. Compared to training algorithms that use multiple models or distinct stages, our approach takes the form of a simple, additional regularization term. It can be interpreted as an inductive version of the classical, transductive label propagation algorithm. We thoroughly evaluate our method on datasets evaluating both synthetic (CIFAR-10, CIFAR-100) and realistic (mini-WebVision, WebVision, Clothing1M, mini-ImageNet-Red) noise, and achieve competitive or state-of-the-art accuracies across all of them.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We show that our method does not perform as well with the synthetic noise in Section~\ref{sec:baselinecomp}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We included a ``Broader impact'' section in the conclusion (Sec.~\ref{sec:conclusion}).}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{The code will be released under Apache License 2.0 upon acceptance. All data is already public.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We included the implementation details in Sec.~\ref{sec:expsetup}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report the standard variation across multiple runs on Tables~\ref{tab:baseline} and~\ref{tab:sota}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We used a single Nvidia V100 GPU for each experiment, as described in Sec.~\ref{sec:expsetup}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
     \answerYes{We use existing, public datasets as described in Sec.~\ref{sec:expsetup}.
        We do not collect any new data for this work.
     }
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> fig_images.tex <==
\begin{figure}
\centering
\begin{tabular}{c c @{~} c @{~} c @{~} c @{~} c}
\toprule
{\bf toucan} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01843383_toucan/clean/00.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01843383_toucan/clean/01.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01843383_toucan/clean/02.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01843383_toucan/clean/03.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01843383_toucan/clean/04.jpg}} \\[10mm]
noise &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01843383_toucan/dirty/00.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01843383_toucan/dirty/01.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01843383_toucan/dirty/02.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01843383_toucan/dirty/03.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01843383_toucan/dirty/04.jpg}} \\[10mm] \toprule  % \\[13mm]
{\bf dugong} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02074367_dugong/clean/00.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02074367_dugong/clean/01.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02074367_dugong/clean/02.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02074367_dugong/clean/03.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02074367_dugong/clean/04.jpg}} \\[10mm]
noise &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02074367_dugong/dirty/00.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02074367_dugong/dirty/01.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02074367_dugong/dirty/02.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02074367_dugong/dirty/03.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02074367_dugong/dirty/04.jpg}} \\[10mm] \toprule  % \\[13mm]
{\bf golden retriever} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02099601_golden_retriever/clean/05.jpg}} & % Do not use 00.jpg, it was used in a previous figure to illustrate a noisy example.
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02099601_golden_retriever/clean/01.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02099601_golden_retriever/clean/02.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02099601_golden_retriever/clean/03.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02099601_golden_retriever/clean/04.jpg}} \\[10mm]
noise &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02099601_golden_retriever/dirty/00.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02099601_golden_retriever/dirty/01.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02099601_golden_retriever/dirty/02.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02099601_golden_retriever/dirty/03.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n02099601_golden_retriever/dirty/04.jpg}} \\[10mm] \toprule  % \\[13mm]
% trifle &
% \raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n07613480_trifle/clean/00.jpg}} &
% \raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n07613480_trifle/clean/01.jpg}} &
% \raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n07613480_trifle/clean/02.jpg}} &
% \raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n07613480_trifle/clean/03.jpg}} &
% \raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n07613480_trifle/clean/04.jpg}} \\
% &
% \raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n07613480_trifle/dirty/00.jpg}} &
% \raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n07613480_trifle/dirty/01.jpg}} &
% \raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n07613480_trifle/dirty/02.jpg}} &
% \raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n07613480_trifle/dirty/03.jpg}} &
% \raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n07613480_trifle/dirty/04.jpg}} \\[10mm] \toprule  % \\[13mm]
{\bf upright piano} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n04515003_upright_piano/clean/00.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n04515003_upright_piano/clean/01.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n04515003_upright_piano/clean/02.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n04515003_upright_piano/clean/03.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n04515003_upright_piano/clean/04.jpg}} \\[10mm]
noise &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n04515003_upright_piano/dirty/00.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n04515003_upright_piano/dirty/01.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n04515003_upright_piano/dirty/02.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n04515003_upright_piano/dirty/03.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n04515003_upright_piano/dirty/04.jpg}} \\[10mm] \toprule  % \\[13mm]
{\bf jellyfish} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01910747_jellyfish/clean/00.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01910747_jellyfish/clean/01.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01910747_jellyfish/clean/02.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01910747_jellyfish/clean/03.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01910747_jellyfish/clean/04.jpg}} \\[10mm]
noise &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01910747_jellyfish/dirty/00.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01910747_jellyfish/dirty/01.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01910747_jellyfish/dirty/02.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01910747_jellyfish/dirty/03.jpg}} &
\raisebox{-0.5\height}{\includegraphics[width=21mm]{fig/dataset_images/imagenet_red/n01910747_jellyfish/dirty/04.jpg}} \\ \bottomrule
\end{tabular}
\caption{Examples with correct (above) and incorrect (below) labels in mini-ImageNet-Red.}
\label{fig:images}
\end{figure}

==> fig_prec_recall.tex <==
\newenvironment{customlegend}[1][]{%
    \begingroup
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%

\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}

\centering
\extdata{fig/data/sample}
\begin{tabular}{@{\xxssp}c@{\xssp}c@{\xxssp}c@{\xxssp}}
\includegraphics[width=0.33\textwidth]{fig/red_twenty_prec_recall.pdf} &
\includegraphics[width=0.33\textwidth]{fig/red_forty_prec_recall.pdf} &
\includegraphics[width=0.33\textwidth]{fig/red_eighty_prec_recall.pdf} \\
a) 20\% Noise Ratio &
b) 40\% Noise Ratio &
c) 80\% Noise Ratio 
\end{tabular}

\centering
\begin{tikzpicture}
\begin{customlegend}[legend columns=4,legend style={align=left,draw=none,column sep=1ex},
        legend entries={Ours + Data Aug. + Mix-Up,
                        Standard,
                        Mix-Up,
                        Data Aug.
                        }]
        \addlegendimage{color=blue, solid, mark=*, mark size=1.5}
        \addlegendimage{color=red, solid, mark=*, mark size=1.5}
        \addlegendimage{color=orange, solid, mark=*, mark size=1.5}
        \addlegendimage{color=gray, solid, mark=*, mark size=1.5}

        \end{customlegend}
\end{tikzpicture}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> plots.tex <==
% main packages
\usepackage{tikz}

\usetikzlibrary{arrows,shapes,calc,matrix,fit,backgrounds}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.9}

% other packages
% \usepackage{chapterfolder}
\usepackage{xstring}

%------------------------------------------------------------------------------
% externalization: requires defining \finalcopy first

\usepgfplotslibrary{external}
% \tikzexternalize
% \tikzexternalize[prefix=fig/extern/]
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\extdata}[1]{\input{#1}}
\IfBeginWith*{\jobname}{fig/extern/}{\finalcopy}{}

%-----------------------------------------------------------------------------
% pgfplots general options

% \newcommand{\plot}[2]{\cffolderinput{#1}{#2}}
% \newcommand{\data}[1]{\cfcurrentfolder #1.txt}
\newcommand{\tabread}[2]{\pgfplotstableread{\data{#1}}#2}

\newcommand{\leg}[1]{\addlegendentry{#1}}
% \newcommand{\legtext}[1]{\addlegendimage{empty legend} \addlegendentry{#1}}

\tikzset{every mark/.append style={solid}}
\pgfplotsset{%smooth,
	grid=both, width=\columnwidth, try min ticks=5,
% 	every axis x label/.style={at={(ticklabel cs:0.5)},anchor=north},
% 	every axis y label/.style={at={(ticklabel cs:0.5)},rotate=90,anchor=south},
	every axis/.append style={font=\scriptsize},
	every axis plot/.append style={thick,mark=none,mark size=1.2,tension=0.18},
	legend cell align=left, legend style={fill opacity=0.8},
}

\pgfplotsset{
	dash/.style={mark=o,dashed,opacity=0.7},
	dott/.style={mark=o,dotted,opacity=0.7},
}
\newcommand{\kilo}[1]{\thisrow{#1}/1000}
\newcommand{\perc}[2]{\thisrow{#1}/#2}
\newcommand{\map}[1]{\thisrow{#1}*100}


==> tables/sota_mini_webvision.tex <==
\begin{table}[tb]
    \centering
    \begin{tabular}{lccccc}
    \toprule
     & ELR \cite{liu2020early} & D-Mix \cite{li2020dividemix} & MOIT \cite{ortego2020multi} & MOIT+~\cite{ortego2020multi} & Ours \\
    \midrule
    Top-1 & 71.9 & 74.6 & 77.8 & 78.7 \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{State-of-the-art comparison on mini-WebVision}}
    \label{tab:sota_mini_webvision}
\end{table}

